Constraining the equation of state of neutron stars using multimessenger observations

Neutron stars are the densest objects known in our visible universe. Properties of matter inside a neutron star are encoded in its equation of state, which has wide-ranging uncertainty from a theoretical perspective. With the current understanding of quantum chromodynamics, it is hard to determine the interactions of neutron star matter at such high densities. Also performing many body calculations is computationally intractable. Besides the constitution of the neutron star core is highly speculative -- it is not ruled out that it contains exotic matter like strange baryons, meson condensates, quark matter, etc. Although the matter inside the neutron star is extremely dense, but the temperature of this object is very cold in most of its life span. We cannot produce such dense but rather cold material in our laboratory. Since probing the physics of neutron star matter is inaccessible by our earth based experiments, we look for astrophysical observations of neutron stars. This thesis deals with the theoretical and computational techniques required to translate neutron star observables from astrophysical observations to its equation of state.

==> cover/certificate_declaration.tex <==
\newgeometry{top=1in,bottom=1in,right=1in,left=1in}
\setboolean{@twoside}{false} 
\chapter*{ Certificate and Declaration}
\addcontentsline{toc}{chapter}{Certificate and Declaration}
%-----------------------------------------------------------------------\\
\markboth{}{}
%\noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}}
%\centerline{\underline{\large\bf Certificate of the Guide}}
\vspace{1.5cm}

\begin{center}
\Large {\textbf{Certificate of the Supervisor}}
\end{center}
This is to certify that the thesis entitled 
 ``{\bf Sources of Stochastic Gravitational Waves and Efficient
Observation with Laser Interferometric Detectors}'' submitted by Mr. Anirban Ain for the award of the degree of Doctor of Philosophy of Jawaharlal Nehru University, New Delhi is his original work. This has not been published or submitted to any other University for any other Degree or Diploma.

\vspace{2cm}

\noindent
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}
Date: & {\bf Prof. Sanjit Mitra} \\
Place:  &    (Thesis Supervisor)
\end{tabular*}


\vspace{2cm}
\begin{center}
\Large {\textbf{Declaration by the Candidate}}
\end{center}
\noindent
I hereby declare that the work reported in this thesis is entirely original. This 
thesis is composed independently by me at the Inter-University Centre for Astronomy and Astrophysics, Pune under the supervision of Prof. Sanjit Mitra. 
I further declare that the subject matter presented in the thesis has not previously formed the basis for the award of any degree, diploma, membership, associateship, fellowship, or any other similar title 
of any University or Institution. 

 
\vspace*{2cm}
\noindent
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}
Date: & {\bf Anirban Ain} \\
Place:  &    (Ph.D. Candidate)
\end{tabular*}

\vspace*{2.5cm}
